Probing the Global Dust Properties and Cluster Formation Potential of the Giant Molecular Cloud G148.24+00.41

Clouds more massive than about $10^5$ M$_\odot$ are potential sites of massive cluster formation. Studying the properties of such clouds in the early stages of their evolution offers an opportunity to test various cluster formation processes. We make use of CO, Herschel, and UKIDSS observations to study one such cloud, G148.24+00.41. Our results show the cloud to be of high mass ($\sim$ $1.1\times10^5$ M$_\odot$), low dust temperature ($\sim$ 14.5 K), nearly circular (projected radius $\sim$ 26 pc), and gravitationally bound with a dense gas fraction of $\sim 18$% and a density profile with a power-law index of $\sim -1.5$. Comparing its properties with those of nearby molecular clouds, we find that G148.24+00.41 is comparable to the Orion-A molecular cloud in terms of mass, size, and dense gas fraction. From our analyses, we find that the central area of the cloud is actively forming protostars and is moderately fractal with a Q-value of $\sim$ 0.66. We also find evidence of global mass-segregation in the cloud, with a degree of mass-segregation ($\Lambda_{MSR}) \approx3.2$. We discuss these results along with the structure and compactness of the cloud, the spatial and temporal distribution of embedded stellar population, and their correlation with the cold dust distribution, in the context of high-mass cluster formation. Comparing our results with models of star cluster formation, we conclude that the cloud has the potential to form a cluster in the mass range $\sim$ 2000--3000 M$_\odot$ through dynamical hierarchical collapse and assembly of both gas and stars.

==> bib.tex <==
\begin{thebibliography}{}
\bibitem[Henshaw et al.(2022)]{henshaw22} Henshaw, J.~D., Barnes, A.~T., Battersby, C., et al.\ 2022, arXiv:2203.11223

\bibitem[Myers(2012)]{mye12} Myers, P.~C.\ 2012, \apj, 752, 9. %doi:10.1088/0004-637X/752/1/9

\bibitem[Kumar et al.(2022)]{kumar22} Kumar, M.~S.~N., Arzoumanian, D., Men'shchikov, A., et al.\ 2022, \aap, 658, A114. %doi:10.1051/0004-6361/202140363


\bibitem[Gutermuth et al.(2008)]{gut08} Gutermuth, R.~A., Bourke, T.~L., Allen, L.~E., et al.\ 2008, \apjl, 673, L151. 
%doi:10.1086/528710

\bibitem[J{\o}rgensen et al.(2006)]{jor06} J{\o}rgensen, J.~K., Harvey, P.~M., Evans, N.~J., et al.\ 2006, \apj, 645, 1246. 
%doi:10.1086/504373

%\bibitem[Hillenbrand \& Hartmann(1998)]{hill98} Hillenbrand, L.~A. \& Hartmann, L.~W.\ 1998, \apj, 492, 540. 
%doi:10.1086/305076


\bibitem[Barentsen et al.(2014)]{bar14} Barentsen, G., Farnhill, H.~J., Drew, J.~E., et al.\ 2014, \mnras, 444, 3230. 
%doi:10.1093/mnras/stu1651

\bibitem[Deharveng et al.(2012)]{deh12} Deharveng, L., Zavagno, A., Anderson, L.~D., et al.\ 2012, \aap, 546, A74. 
%doi:10.1051/0004-6361/201219131


\bibitem[Planck Collaboration et al.(2011)]{pla11a} Planck Collaboration, Ade, P.~A.~R., Aghanim, N., et al.\ 2011, \aap, 536, A1. 
%doi:10.1051/0004-6361/201116464

\bibitem[Myers(2009)]{mye09} Myers, P.~C.\ 2009, \apj, 700, 1609. %doi:10.1088/0004-637X/700/2/1609


\bibitem[G{\'o}mez \& V{\'a}zquez-Semadeni(2014)]{gom14} G{\'o}mez, G.~C. \& V{\'a}zquez-Semadeni, E.\ 2014, \apj, 791, 124. %doi:10.1088/0004-637X/791/2/124


\bibitem[Planck Collaboration et al.(2011)]{pla11} Planck Collaboration, Ade, P.~A.~R., Aghanim, N., et al.\ 2011, \aap, 536, A7.


\bibitem[Bolatto et al.(2008)]{bal08} Bolatto, A.~D., Leroy, A.~K., Rosolowsky, E., et al.\ 2008, \apj, 686, 948.

\bibitem[Barnes et al.(2019)]{barnes_2019} Barnes A.~T., Longmore S.~N., Avison A., Contreras Y., Ginsburg A., Henshaw J.~D., Rathborne J.~M., et al., 2019, MNRAS, 486, 283.


\bibitem[He et al.(2022)]{he22} He, H., Wilson, C., Brunetti, N., et al.\ 2022, \apj, 928, 57. 


\bibitem[Hacar et al.(2022)]{hac22} Hacar, A., Clark, S., Heitsch, F., et al.\ 2022, arXiv:2203.09562.

\bibitem[Pineda et al.(2022)]{pin22} Pineda, J.~E., Arzoumanian, D., Andr{\'e}, P., et al.\ 2022, arXiv:2205.03935.


%\bibitem[Matzner \& Jumper(2015)]{mat15} Matzner, C.~D. \& Jumper, P.~H.\ 2015, \apj, 815, 68.


\bibitem[Montillaud et al.(2019)]{mon19} Montillaud, J., Juvela, M., Vastel, C., et al.\ 2019, \aap, 631, A3. 


\bibitem[Trevi{\~n}o-Morales et al.(2019)]{tre19} Trevi{\~n}o-Morales, S.~P., Fuente, A., S{\'a}nchez-Monge, {\'A}., et al.\ 2019, \aap, 629, A81. 



\bibitem[Krause et al.(2020)]{kra20} Krause, M.~G.~H., Offner, S.~S.~R., Charbonnel, C., et al.\ 2020, \ssr, 216, 64.


\bibitem[Dobbs et al.(2005)]{dobb05} Dobbs, C.~L., Bonnell, I.~A., \& Clark, P.~C.\ 2005, \mnras, 360, 2. 

\bibitem[Maschberger et al.(2010)]{mas10} Maschberger, T., Clarke, C.~J., Bonnell, I.~A., et al.\ 2010, \mnras, 404, 1061. 

\bibitem[V{\'a}zquez-Semadeni et al.(2019)]{vaz19} V{\'a}zquez-Semadeni, E., Palau, A., Ballesteros-Paredes, J., et al.\ 2019, \mnras, 490, 3061.



\bibitem[Karam \& Sills(2022)]{karam22} Karam, J. \& Sills, A.\ 2022, \mnras, 513, 6095. 


\bibitem[Sills et al.(2018)]{sills18} Sills, A., Rieder, S., Scora, J., et al.\ 2018, \mnras, 477, 1903. 


\bibitem[Yadav et al.(2022)]{yad22} Yadav, R.~K., Samal, M.~R., Semenko, E., et al.\ 2022, \apj, 926, 16. 



\bibitem[Walker et al.(2015)]{walk15} Walker, D.~L., Longmore, S.~N., Bastian, N., et al.\ 2015, \mnras, 449, 715. 

\bibitem[Parker et al.(2016)]{park16} Parker, R.~J., Goodwin, S.~P., Wright, N.~J., et al.\ 2016, \mnras, 459, L119. 


\bibitem[Clark \& Whitworth(2021)]{clark21} Clark, P.~C. \& Whitworth, A.~P.\ 2021, \mnras, 500, 1697.


\bibitem[Li(2018)]{li18} Li, G.-X.\ 2018, \mnras, 477, 4951.


\bibitem[Donkov \& Stefanov(2018)]{don18} Donkov, S. \& Stefanov, I.~Z.\ 2018, \mnras, 474, 5588. 



\bibitem[Spilker et al.(2021)]{spi21} Spilker, A., Kainulainen, J., \& Orkisz, J.\ 2021, \aap, 653, A63. 


\bibitem[Marsh \& Whitworth(2019)]{mar19} Marsh, K.~A. \& Whitworth, A.~P.\ 2019, \mnras, 483, 352. 


\bibitem[Wenger et al.(2018)]{weng18} Wenger, T.~V., Balser, D.~S., Anderson, L.~D., et al.\ 2018, \apj, 856, 52. 


\bibitem[Su et al.(2019)]{su19} Su, Y., Yang, J., Zhang, S., et al.\ 2019, \apjs, 240, 9.


\bibitem[Winston et al.(2019)]{wins19} Winston, E., Hora, J., Gutermuth, R., et al.\ 2019, \apj, 880, 9. 



\bibitem[Maud et al.(2015)]{maud15} Maud, L.~T., Moore, T.~J.~T., Lumsden, S.~L., et al.\ 2015, \mnras, 453, 645. 


\bibitem[Lumsden et al.(2013)]{lums13} Lumsden, S.~L., Hoare, M.~G., Urquhart, J.~S., et al.\ 2013, \apjs, 208, 11. 


\bibitem[Chevance et al.(2022)]{che22} Chevance, M., Krumholz, M.~R., McLeod, A.~F., et al.\ 2022, arXiv:2203.09570.

\bibitem[Krumholz \& McKee(2020)]{krum20} Krumholz, M.~R. \& McKee, C.~F.\ 2020, \mnras, 494, 624.

%\bibitem[Krumholz et al.(2019)]{krum19} Krumholz, M.~R., McKee, C.~F., \& Bland-Hawthorn, J.\ 2019, \araa, 57, 227. 

\bibitem[Longmore et al.(2014)]{long14} Longmore, S.~N., Kruijssen, J.~M.~D., Bastian, N., et al.\ 2014, Protostars and Planets VI, 291.

\bibitem[Geen et al.(2015)]{green15} Green, S., Hennebelle, P., Tremblin, P., et al.\ 2015, \mnras, 454, 4484. 

\bibitem[Geen et al.(2016)]{green16} Geen, S., Hennebelle, P., Tremblin, P., et al.\ 2016, \mnras, 463, 3129. 

\bibitem[Kim et al.(2018)]{kim18} Kim, J.-G., Kim, W.-T., \& Ostriker, E.~C.\ 2018, \apj, 859, 68. 


\bibitem[Banerjee \& Kroupa(2018)]{ban18} Banerjee, S. \& Kroupa, P.\ 2018, The Birth of Star Clusters, 424, 143. 

\bibitem[Banerjee \& Kroupa(2015)]{ban15} Banerjee, S. \& Kroupa, P.\ 2015, \mnras, 447, 728. 


\bibitem[Dobbs et al.(2011)]{dobbs11} Dobbs, C.~L., Burkert, A., \& Pringle, J.~E.\ 2011, \mnras, 413, 2935.


\bibitem[MacLaren et al.(1988)]{MacLaren1988}
MacLaren, I., Richardson, K.~M., \& Wolfendale, A.~W.\ 1988, \apj, 333, 821.


\bibitem[Dobbs et al.(2011)]{dobb11} Dobbs, C.~L., Burkert, A., \& Pringle, J.~E.\ 2011, \mnras, 413, 2935.


\bibitem[Garay et al.(2007)]{gary07} Garay, G., Mardones, D., Brooks, K.~J., et al.\ 2007, \apj, 666, 309. 

\bibitem[Chen et al.(2021)]{chen21} Chen, Y., Li, H., \& Vogelsberger, M.\ 2021, \mnras, 502, 6157. 



\bibitem[Zari et al.(2016)]{zari16} Zari, E., Lombardi, M., Alves, J., Lada, C.~J., \& Bouy, H.\ 2016, \aap, 587, A106.

\bibitem[Lombardi et al.(2014)]{lom14} Lombardi, M., Bouy, H., Alves, J., \& Lada, C.~J.\ 2014, \aap, 566, A45.

\bibitem[Lombardi et al.(2013)]{lom13} Lombardi, M., Lada, C.~J., \& Alves, J.\ 2013, \aap, 559, A90.

\bibitem[Lombardi et al.(2010)]{lom10} Lombardi, M., Alves, J., \& Lada, C.~J.\ 2010, \aap, 519, L7.

\bibitem[Howard et al.(2018)]{how18} Howard, C.~S., Pudritz, R.~E., \& Harris, W.~E.\ 2018, Nature Astronomy, 2, 725.


\bibitem[Gavagnin et al.(2017)]{gav17} Gavagnin, E., Bleuler, A., Rosdahl, J., \& Teyssier, R.\ 2017, \mnras, 472, 4155.


\bibitem[Miville-Desch{\^e}nes et al.(2017)]{mivi17} Miville-Desch{\^e}nes, M.-A., Murray, N., \& Lee, E.~J.\ 2017, \apj, 834, 57.

\bibitem[Yang et al.(2002)]{yang02} Yang, J., Jiang, Z., Wang, M., Ju, B., \& Wang, H.\ 2002, \apjs, 141, 157.

\bibitem[Zhang et al.(2018)]{zhag18} Zhang, C.-P., Liu, T., Yuan, J., et al.\ 2018, \apjs, 236, 49.

\bibitem[Yuan et al.(2016)]{yuan16} Yuan, J., Wu, Y., Liu, T., et al.\ 2016, \apj, 820, 37.

\bibitem[Cooper et al.(2013)]{coop13} Cooper, H.~D.~B., Lumsden, S.~L., Oudmaijer, R.~D., et al.\ 2013, \mnras, 430, 1125.


\bibitem[Andr{\'e} et al.(2010)]{and10} Andr{\'e}, P., Men'shchikov, A., Bontemps, S., et al.\ 2010, \aap, 518, L102.



\bibitem[Peretto et al.(2013)]{per13} Peretto, N., Fuller, G.~A., Duarte-Cabral, A., et al.\ 2013, \aap, 555, A112.



\bibitem[Dutta et al.(2018)]{dut18} Dutta, S., Mondal, S., Samal, M.~R., \& Jose, J.\ 2018, \apj, 864, 154.


\bibitem[Ryabukhina et al.(2018)]{rya18} Ryabukhina, O.~L., Zinchenko, I.~I., Samal, M.~R., et al.\ 2018, Research in Astronomy and Astrophysics, 18, 095.


\bibitem[Heyer et al.(2009)]{hey09} Heyer, M., Krawczyk, C., Duval, J., \& Jackson, J.~M.\ 2009, \apj, 699, 1092.


\bibitem[Marsh et al.(2015)]{mar15} Marsh, K.~A., Whitworth, A.~P., \& Lomax, O.\ 2015, \mnras, 454, 428.


\bibitem[Murray \& Chang(2015)]{mur15} Murray, N., \& Chang, P.\ 2015, \apj, 804, 44.


\bibitem[Solomon et al.(1987)]{sol87} Solomon, P.~M., Rivolo, A.~R., Barrett, J., \& Yahil, A.\ 1987, \apj, 319, 730.


\bibitem[Evans et al.(2014)]{evans14} Evans, N.~J., II, Heiderman, A., \& Vutisalchavakul, N.\ 2014, \apj, 782, 114.


\bibitem[Andr{\'e} et al.(2014)]{andre14}
Andr{\'e}, P., Di Francesco, J., Ward-Thompson, D., et al. 2014, in Protostars and Planets VI, ed. H. Beuther et al. (Tucson, AZ; Univ. Arizona Press), 27.



\bibitem[Andr{\'e} et al.(2016)]{andre2016} Andr{\'e} P., K{\"o}nyves V., Roy A., Arzoumanian D., 2016, IAUFM, 29B, 708.



\bibitem[Bohlin et al.(1978)]{bohlin78}
Bohlin, R.~C., Savage, B.~D., \& Drake, J.~F. 1978, ApJ, 224, 13233.



\bibitem[Evans et al.(2009)]{evans09}
Evans, N.~J., II, Dunham, M.~M., J\o{}rgensen, J.~K., et al. 2009, ApJS, 181, 321.



\bibitem[Lawrence et al.(2007)]{lawrence07}
Lawrence, A., Warren, S.~J., Almaini, O., et al. 2007, MNRAS, 379, 1599.



\bibitem[Allison et al.(2010)]{alli10} Allison, R.~J., Goodwin, S.~P., Parker, R.~J., Portegies Zwart, S.~F., \& de Grijs, R.\ 2010, \mnras, 407, 1098.


\bibitem[Kauffmann et al.(2008)]{kauffmann2008} Kauffmann J., Bertoldi F., Bourke T.~L., Evans N.~J., Lee C.~W., 2008, A\&A, 487, 993.

\bibitem[Kauffmann \& Pillai(2010)]{kauffmann_pillai2010} Kauffmann J., Pillai T., 2010, ApJL, 723, L7.


\bibitem[Lada, Lombardi, \& Alves(2010)]{lada2010} Lada C.~J., Lombardi M., Alves J.~F., 2010, ApJ, 724, 687.


\bibitem[Lucas et al.(2008)]{lucas2008} Lucas P.~W., Hoare M.~G., Longmore A., Schr{\"o}der A.~C., Davis C.~J., Adamson A., Bandyopadhyay R.~M., et al., 2008, MNRAS, 391, 136.

  


\bibitem[Zamora-Avil{\'e}s et al.(2012)]{zamora12} Zamora-Avil{\'e}s, M., V{\'a}zquez-Semadeni, E., \& Col{\'{\i}}n, P.\ 2012, \apj, 751, 77.


\bibitem[Portegies Zwart et al.(2010)]{por10} Portegies Zwart, S.~F., McMillan, S.~L.~W., \& Gieles, M.\ 2010, \araa, 48, 431.





\bibitem[V{\'a}zquez-Semadeni et al.(2009)]{vaz09} V{\'a}zquez-Semadeni, E., G{\'o}mez, G.~C., Jappsen, A.-K., Ballesteros-Paredes, J., \& Klessen, R.~S.\ 2009, \apj, 707, 1023.


\bibitem[Lada \& Lada(2003)]{lada03} Lada, C.~J., \& Lada, E.~A.\ 2003, \araa, 41, 57.



%\bibitem[Samal et al.(2018)]{samal18} Samal, M.~R., Deharveng, L., Zavagno, A., et al.\ 2018, \aap, 617, A67.



\bibitem[Deharveng et al.(2015)]{deh15} Deharveng, L., Zavagno, A., Samal, M.~R., et al.\ 2015, \aap, 582, A1.



\bibitem[Bressan et al.(2012)]{bre12} Bressan, A., Marigo, P., Girardi, L., et al.\ 2012, \mnras, 427, 127.


%\bibitem[Ojha et al.(2011)]{ojha11} Ojha, D.~K., Samal, M.~R., Pandey, A.~K., et al.\ 2011, \apj, 738, 156.


\bibitem[Rieke \& Lebofsky(1985)]{rie85} Rieke, G.~H., \& Lebofsky, M.~J.\ 1985, \apj, 288, 618.

\bibitem[Lada et al.(2012)]{lada12} Lada, C.~J., Forbrich, J., Lombardi, M., \& Alves, J.~F.\ 2012, \apj, 745, 190.



\bibitem[Heiderman et al.(2010)]{hei10} Heiderman, A., Evans, N.~J., II, Allen, L.~E., Huard, T., \& Heyer, M.\ 2010, \apj, 723, 1019.



\bibitem[Marsh et al.(2017)]{marsh17} Marsh, K.~A., Whitworth, A.~P., Lomax, O., et al.\ 2017, \mnras, 471, 2730.



\bibitem[Dobashi et al.(2005)]{dob05} Dobashi K., Uehara H., Kandori R., Sakurai T., Kaiden M., Umemoto T., Sato F., 2005, PASJ, 57, S1.

\bibitem[Dobashi (2011)]{dob11} Dobashi K., 2011, PASJ, 63, S1.

\bibitem[Wouterloot \& Brand (1989)]{wb1989} Wouterloot J.~G.~A., Brand J., 1989, LNP, 97.


\bibitem[Reid et al.(2019)]{reid_2019} Reid M.~J., Menten K.~M., Brunthaler A., Zheng X.~W., Dame T.~M., Xu Y., Li J., et al., 2019, ApJ, 885, 131.


\bibitem[Molinari et al.(2010a)]{Mol_2010a} Molinari S., Swinyard B., Bally J., Barlow M., Bernard J.-P., Martin P., Moore T., et al., 2010, A\&A, 518, L100.

%\bibitem[Molinari et al.(2010b)]{Mol_2010b} Molinari S., Swinyard B., Bally J., Barlow M., Bernard J.-P., Martin P., Moore T., et al., 2010, PASP, 122, 314.


\bibitem[Kauffmann et al.(2017)]{kauff2017} Kauffmann J., Pillai T., Zhang Q., Menten K.~M., Goldsmith P.~F., Lu X., Guzm{\'a}n A.~E., 2017, A\&A, 603, A89.

\bibitem[Rathborne et al.(2015)]{rath2015} Rathborne J.~M., Longmore S.~N., Jackson J.~M., Alves J.~F., Bally J., Bastian N., Contreras Y., et al., 2015, ApJ, 802, 125.

\bibitem[Walker et al.(2016)]{walker2016} Walker D.~L., Longmore S.~N., Bastian N., Kruijssen J.~M.~D., Rathborne J.~M., Galv{\'a}n-Madrid R., Liu H.~B., 2016, MNRAS, 457, 4536.


\bibitem[Walker et al.(2018)]{walker2018} Walker D.~L., Longmore S.~N., Zhang Q., Battersby C., Keto E., Kruijssen J.~M.~D., Ginsburg A., et al., 2018, MNRAS, 474, 2373.

%\bibitem[Green et al.(2019)]{gre19} Green G.~M., Schlafly E., Zucker C., Speagle J.~S., Finkbeiner D., 2019, ApJ, 887, 93.

\bibitem[Herschel Point Source Catalogue Working Group et al.(2020)]{hers2020} Herschel Point Source Catalogue Working Group, Marton G., Calzoletti L., Perez Garcia A.~M., Kiss C., Paladini R., Altieri B., et al., 2020, yCat, VIII/106.

\bibitem[Marton et al.(2017)]{mart2017} Marton G., Calzoletti L., Perez Garcia A.~M., Kiss C., Paladini R., Altieri B., Sanchez Portal M., et al., 2017, arXiv, arXiv:1705.05693.

\bibitem[Furlan et al.(2016)]{fur2016} Furlan E., Fischer W.~J., Ali B., Stutz A.~M., Stanke T., Tobin J.~J., Megeath S.~T., et al., 2016, ApJS, 224, 5.

\bibitem[Cartwright \& Whitworth(2004)]{cart-whit2004} Cartwright A., Whitworth A.~P., 2004, MNRAS, 348, 589.

\bibitem[Schmeja \& Klessen(2006)]{sch-kle2006} Schmeja S., Klessen R.~S., 2006, A\&A, 449, 151.

\bibitem[Parker et al.(2014)]{park2014} Parker R.~J., Wright N.~J., Goodwin S.~P., Meyer M.~R., 2014, MNRAS, 438, 620.

\bibitem[Sanhueza et al.(2019)]{san2019} Sanhueza P., Contreras Y., Wu B., Jackson J.~M., Guzm{\'a}n A.~E., Zhang Q., Li S., et al., 2019, ApJ, 886, 102.

\bibitem[Dib \& Henning(2019)]{dib-hen2019} Dib S., Henning T., 2019, A\&A, 629, A135.

\bibitem[Gouliermis et al.(2012)]{goul2012} Gouliermis D.~A., Schmeja S., Dolphin A.~E., Gennaro M., Tognelli E., Prada Moroni P.~G., 2012, ApJ, 748, 64.


\bibitem[Dunham et al.(2008)]{dun2008} Dunham M.~M., Crapsi A., Evans N.~J., Bourke T.~L., Huard T.~L., Myers P.~C., Kauffmann J., 2008, ApJS, 179, 249.

\bibitem[Ragan et al.(2012)]{rag2012} Ragan S., Henning T., Krause O., Pitann J., Beuther H., Linz H., Tackenberg J., et al., 2012, A\&A, 547, A49.

\bibitem[Commer{\c{c}}on et al.(2012)]{com2012} Commer{\c{c}}on B., Launhardt R., Dullemond C., Henning T., 2012, A\&A, 545, A98.

\bibitem[Samal et al.(2018)]{samal2018} Samal M.~R., Chen W.~P., Takami M., Jose J., Froebrich D., 2018, MNRAS, 477, 4577.

\bibitem[Dom{\'\i}nguez et al.(2017)]{dom2017} Dom{\'\i}nguez R., Fellhauer M., Bla{\~n}a M., Farias J.~P., Dabringhausen J., 2017, MNRAS, 472, 465.

\bibitem[Foster et al.(2015)]{fost2015} Foster, J.~B. and 16 colleagues 2015.\ IN-SYNC. II. Virial Stars from Subvirial Cores{\textemdash}the Velocity Dispersion of Embedded Pre-main-sequence Stars in NGC 1333.\ The Astrophysical Journal 799.

\bibitem[Allison et al.(2009)]{ali2009} Allison R.~J., Goodwin S.~P., Parker R.~J., Portegies Zwart S.~F., de Grijs R., Kouwenhoven M.~B.~N., 2009, MNRAS, 395, 1449.

\bibitem[Maschberger \& Clarke(2011)]{mas-clark2011} Maschberger T., Clarke C.~J., 2011, MNRAS, 416, 541.

\bibitem[Plunkett et al.(2018)]{plunk2018} Plunkett A.~L., Fern{\'a}ndez-L{\'o}pez M., Arce H.~G., Busquet G., Mardones D., Dunham M.~M., 2018, A\&A, 615, A9.

\bibitem[Sadaghiani et al.(2020)]{sad2020} Sadaghiani M., S{\'a}nchez-Monge {\'A}., Schilke P., Liu H.~B., Clarke S.~D., Zhang Q., Girart J.~M., et al., 2020, A\&A, 635, A2.

\bibitem[Meingast, Lombardi, \& Alves(2017)]{mein2017} Meingast S., Lombardi M., Alves J., 2017, A\&A, 601, A137.

\bibitem[Larson(1981)]{lar1981} Larson R.~B., 1981, MNRAS, 194, 809.

\bibitem[Dunham et al.(2006)]{dun2006} Dunham M.~M., Evans N.~J., Bourke T.~L., Dullemond C.~P., Young C.~H., Brooke T.~Y., Chapman N., et al., 2006, ApJ, 651, 945.

\bibitem[Bonnell \& Bate(2006)]{bon-bate2006} Bonnell I.~A., Bate M.~R., 2006, MNRAS, 370, 488. 

\bibitem[Girichidis et al.(2012)]{gir2012} Girichidis P., Federrath C., Banerjee R., Klessen R.~S., 2012, MNRAS, 420, 613.

%\bibitem[Heyer, Carpenter, \& Snell(2001)]{hey-car-snell2001} Heyer M.~H., Carpenter J.~M., Snell R.~L., 2001, ApJ, 551, 852.

\bibitem[Clark et al.(2005)]{clark2005} Clark P.~C., Bonnell I.~A., Zinnecker H., Bate M.~R., 2005, MNRAS, 359, 809.

\bibitem[Clark \& Bonnell(2004)]{clark-bon2004} Clark P.~C., Bonnell I.~A., 2004, MNRAS, 347, L36.

\bibitem[Bertoldi \& McKee(1992)]{ber-mck1992} Bertoldi F., McKee C.~F., 1992, ApJ, 395, 140.

\bibitem[Mao, Ostriker, \& Kim(2020)]{mao2020} Mao S.~A., Ostriker E.~C., Kim C.-G., 2020, ApJ, 898, 52.

\bibitem[Weidner, Kroupa, \& Bonnell(2010)]{weid2010} Weidner C., Kroupa P., Bonnell I.~A.~D., 2010, MNRAS, 401, 275.

\bibitem[Baldeschi et al.(2017)]{bald2017} Baldeschi A., Elia D., Molinari S., Pezzuto S., Schisano E., Gatti M., Serra A., et al., 2017, MNRAS, 466, 3682.

\bibitem[Caldwell \& Chang(2018)]{cald-chan2018} Caldwell S., Chang P., 2018, MNRAS, 474, 4818.

\bibitem[Lee, Miville-Desch{\^e}nes, \& Murray(2016)]{lee2016} Lee E.~J., Miville-Desch{\^e}nes M.-A., Murray N.~W., 2016, ApJ, 833, 229.

\bibitem[Bastian \& Goodwin(2006)]{bast2006} Bastian N., Goodwin S.~P., 2006, MNRAS, 369, L9.

\bibitem[Smith, Longmore, \& Bonnell(2009)]{smith2009} Smith R.~J., Longmore S., Bonnell I., 2009, MNRAS, 400, 1775.

\bibitem[Longmore et al.(2014)]{long2014} Longmore S.~N., Kruijssen J.~M.~D., Bastian N., Bally J., Rathborne J., Testi L., Stolte A., et al., 2014, prpl.conf, 291.

\bibitem[Krumholz \& McKee(2020)]{krum-mck2020} Krumholz M.~R., McKee C.~F., 2020, MNRAS, 494, 624. 

\bibitem[Padoan et al.(2020)]{pad2020} Padoan P., Pan L., Juvela M., Haugb{\o}lle T., Nordlund {\r{A}}., 2020, ApJ, 900, 82. 

\bibitem[Winston, Hora, \& Tolls(2020)]{wins2020} Winston E., Hora J.~L., Tolls V., 2020, AJ, 160, 68. 

\bibitem[Pfalzner(2009)]{pfal2009} Pfalzner S., 2009, A\&A, 498, L37. 

\bibitem[Ochsenbein, Bauer, \& Marcout(2000)]{viz2000} Ochsenbein F., Bauer P., Marcout J., 2000, A\&AS, 143, 23.

\bibitem[Elmegreen \& Efremov(1997)]{elm-efre_1997} Elmegreen B.~G., Efremov Y.~N., 1997, ApJ, 480, 235.

\bibitem[Urquhart et al.(2008)]{urqh_2008} Urquhart J.~S., Busfield A.~L., Hoare M.~G., Lumsden S.~L., Oudmaijer R.~D., Moore T.~J.~T., Gibb A.~G., et al., 2008, A\&A, 487, 253.

\bibitem[Henshaw et al.(2022)]{Hen_2022} Henshaw J.~D., Barnes A.~T., Battersby C., Ginsburg A., Sormani M.~C., Walker D.~L., 2022, arXiv, arXiv:2203.11223

\bibitem[Kroupa(2001)]{kroupa_2001} Kroupa P., 2001, MNRAS, 322, 231.

\bibitem[Whitney \& GLIMPSE360 Team(2009)]{whit_glimpse_2009} Whitney B., GLIMPSE360 Team, 2009, AAS

\bibitem[Walker et al.(2016)]{walk_2016} Walker D.~L., Longmore S.~N., Bastian N., Kruijssen J.~M.~D., Rathborne J.~M., Galv{\'a}n-Madrid R., Liu H.~B., 2016, MNRAS, 457, 4536.

\bibitem[Weisz et al.(2015)]{wei_15} Weisz, D.~R., Johnson, L.~C., Foreman-Mackey, D., et al.\ 2015, \apj, 806, 198. doi:10.1088/0004-637X/806/2/198

\nocite{*}
% Alternatively you could enter them by hand, like this:
% This method is tedious and prone to error if you have lots of references
%\begin{thebibliography}{99}
%\bibitem[\protect\citeauthoryear{Author}{2012}]{Author2012}
%Author A.~N., 2013, Journal of Improbable Astronomy, 1, 1
%\bibitem[\protect\citeauthoryear{Others}{2013}]{Others2013}
%Others S., 2012, Journal of Interesting Stuff, 17, 198
\end{thebibliography}
